On the application of simplified rheological models of fluid in the hydraulic fracture problems

In this paper we analyse a problem of a hydraulic fracture driven by a non-Newtonian shear-thinning fluid. For the PKN fracture geometry we consider three different rheological models of fluid: i) the Carreau fluid, ii) the truncated power-law fluid, iii) the power-law fluid. For each of these models a number of simulations are performed. The results are post-processed and compared with each other in order to find decisive factors for similarities/dissimilarities. It is shown that under certain conditions even the basic power-law rheology can be a good substitute for the Carreau characteristics. Although for a particular fluid such a conclusion cannot be made a priori, post-processing based on average values of the fluid shear rates is a very good tool to verify credibility of the results obtained for simplified rheological models. The truncated power-law rheology is a good alternative for the Carreau model. It always produces results that are very similar to those obtained with the equivalent Carreau fluid and simultaneously provides a relative ease of numerical implementation.

==> definitions.tex <==
%Definitions: general
\newcommand{\singlespace}{\baselineskip=12pt \lineskiplimit=0pt \lineskip=0pt}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\lb}{\label}
\newcommand{\beqar}{\begin{eqnarray}}
\newcommand{\eeqar}{\end{eqnarray}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
\newcommand{\barr}{\begin{array}}
\newcommand{\earr}{\end{array}}
\def\ds{\displaystyle}
\newcommand\eq[1]{(\ref{#1})}
\newcommand{\bfm}[1]{\mbox{\boldmath ${#1}$}}        % produces bold math symbol

%Definitions: theorem
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{remark}{Remark}[section]
% \newtheorem{corollary}{Corollary}[section]

%Definitions: symbols
% \newcommand{\jump}[2]{[\mbox{\hspace{-#1em}}[#2]\mbox{\hspace{-#1em}}]}
% dopodiche' scrivi il comando
% \jump{*}{**}
% dove * e' un numero mentre ** e' quello che tu vuoi tra parentesi.
% Il numero serve a far si che le due parentesi quadre che comporranno
% l'unica parentesi che tu vuoi siano ben posizionate. Tale numero varia a
% seconda di chi sia **.

% \newcommand{\bjump}[2]{\left[\mbox{\hspace{-#1em}}\left[#2\right]\mbox{\hspace{-#1em}}\right]}
% con parentesi di altezza variabile

\def\scalp{\mbox{\boldmath $\, \cdot \,$}}
\def\bob{{\, \underline{\overline{\otimes}} \,}}
%\def\bob{\makebox{\raisebox{-.215ex}{$\Box$}\hspace{-.73em}$\scalp$}}
\def\gdp{\ \begin{picture}
           (6,6)\put(0,0){\framebox(6,6){$\times$}}
           \end{picture} \ }
%\def\gdp{\makebox{\raisebox{-.215ex}{$\Box$}\hspace{-.778em}$\times$}}
\def\sop{{\, \overline{\otimes} \,}}
\def\sot{{\, \underline{\otimes} \,}}
\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\nderiv}[3]{\frac{\partial^{\,#3} #1}{\partial #2^{\,#3}}}
\newcommand{\maxx}[2]{\text{Max}_{#1}\ \left(#2\right)}
\newcommand{\oldr}[1]{\stackrel{\circ}{\mbox{#1}}}
%\newcommand{\pv}{-\mskip-19mu\int}
\newcommand{\modI}{\text{I}}
\newcommand{\modII}{\text{II}}
\newcommand{\modIII}{\text{III}}
\def\Xint#1{\mathchoice
   {\XXint\displaystyle\textstyle{#1}}%
   {\XXint\textstyle\scriptstyle{#1}}%
   {\XXint\scriptstyle\scriptscriptstyle{#1}}%
   {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
   \!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
   \vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\fp{\Xint=}
\def\pv{\Xint-}

%Definitions: vectors and points and second-order tensor
\def\b0{\mbox{\boldmath $0$}}
\def\ba{\mbox{\boldmath $a$}}
\def\bb{\mbox{\boldmath $b$}}
\def\bc{\mbox{\boldmath $c$}}
\def\bd{\mbox{\boldmath $d$}}
\def\be{\mbox{\boldmath $e$}}
\def\beffe{\mbox{\boldmath $f$}}
\def\bg{\mbox{\boldmath $g$}}
\def\bh{\mbox{\boldmath $h$}}
\def\bi{\mbox{\boldmath $i$}}
\def\bj{\mbox{\boldmath $j$}}
\def\bk{\mbox{\boldmath $k$}}
\def\bl{\mbox{\boldmath $l$}}
\def\bm{\mbox{\boldmath $m$}}
\def\bn{\mbox{\boldmath $n$}}
\def\bo{\mbox{\boldmath $o$}}
\def\bp{\mbox{\boldmath $p$}}
\def\bq{\mbox{\boldmath $q$}}
\def\br{\mbox{\boldmath $r$}}
\def\bs{\mbox{\boldmath $s$}}
\def\bt{\mbox{\boldmath $t$}}
\def\bu{\mbox{\boldmath $u$}}
\def\bv{\mbox{\boldmath $v$}}
\def\bw{\mbox{\boldmath $w$}}
\def\bx{\mbox{\boldmath $x$}}
\def\by{\mbox{\boldmath $y$}}
\def\bz{\mbox{\boldmath $z$}}
\def\bA{\mbox{\boldmath $A$}}
\def\bB{\mbox{\boldmath $B$}}
\def\bC{\mbox{\boldmath $C$}}
\def\bD{\mbox{\boldmath $D$}}
\def\bE{\mbox{\boldmath $E$}}
\def\bF{\mbox{\boldmath $F$}}
\def\bG{\mbox{\boldmath $G$}}
\def\bH{\mbox{\boldmath $H$}}
\def\bI{\mbox{\boldmath $I$}}
\def\bJ{\mbox{\boldmath $J$}}
\def\bK{\mbox{\boldmath $K$}}
\def\bL{\mbox{\boldmath $L$}}
\def\bM{\mbox{\boldmath $M$}}
\def\bN{\mbox{\boldmath $N$}}
\def\bO{\mbox{\boldmath $O$}}
\def\bP{\mbox{\boldmath $P$}}
\def\bQ{\mbox{\boldmath $Q$}}
\def\bR{\mbox{\boldmath $R$}}
\def\bS{\mbox{\boldmath $S$}}
\def\bT{\mbox{\boldmath $T$}}
\def\bU{\mbox{\boldmath $U$}}
\def\bV{\mbox{\boldmath $V$}}
\def\bW{\mbox{\boldmath $W$}}
\def\bX{\mbox{\boldmath $X$}}
\def\bY{\mbox{\boldmath $Y$}}
\def\bZ{\mbox{\boldmath $Z$}}

\def\Id{\mbox{\boldmath $I$}}
\newcommand{\bsigma}{\mbox{\boldmath $\sigma$}}
\newcommand{\bSigma}{\mbox{\boldmath $\Sigma$}}
\newcommand{\bepsilon}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bvarepsilon}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\btau}{\mbox{\boldmath $\tau$}}
\newcommand{\bpsi}{\mbox{\boldmath$\psi$}}
\newcommand{\bPsi}{\mbox{\boldmath$\Psi$}}
\newcommand{\bxi}{\mbox{\boldmath $\xi$}}
\newcommand{\bphi}{\mbox{\boldmath $\phi$}}
\newcommand{\bvarphi}{\mbox{\boldmath$\varphi$}}
\newcommand{\bPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\bXi}{\mbox{\boldmath $\Xi$}}
\newcommand{\bchi}{\mbox{\boldmath $\chi$}}
\newcommand{\bmu}{\mbox{\boldmath $\mu$}}

%Definitions: fourth-order tensors
\def\f0{\ensuremath{\mathbb{O}}}
\def\fA{\ensuremath{\mathbb{A}}}
\def\fB{\ensuremath{\mathbb{B}}}
\def\fC{\ensuremath{\mathbb{C}}}
\def\fD{\ensuremath{\mathbb{D}}}
\def\fE{\ensuremath{\mathbb{E}}}
\def\fF{\ensuremath{\mathbb{F}}}
\def\fG{\ensuremath{\mathbb{G}}}
\def\fH{\ensuremath{\mathbb{H}}}
\def\fI{\ensuremath{\mathbb{I}}}
\def\fJ{\ensuremath{\mathbb{J}}}
\def\fK{\ensuremath{\mathbb{K}}}
\def\fL{\ensuremath{\mathbb{L}}}
\def\fM{\ensuremath{\mathbb{M}}}
\def\fN{\ensuremath{\mathbb{N}}}
\def\fO{\ensuremath{\mathbb{O}}}
\def\fP{\ensuremath{\mathbb{P}}}
\def\fQ{\ensuremath{\mathbb{Q}}}
\def\fR{\ensuremath{\mathbb{R}}}
\def\fS{\ensuremath{\mathbb{S}}}
\def\fT{\ensuremath{\mathbb{T}}}
\def\fU{\ensuremath{\mathbb{U}}}
\def\fV{\ensuremath{\mathbb{V}}}
\def\fW{\ensuremath{\mathbb{W}}}
\def\fX{\ensuremath{\mathbb{X}}}
\def\fY{\ensuremath{\mathbb{Y}}}
\def\fZ{\ensuremath{\mathbb{Z}}}

% Abbreviate definitions of greek symbols
\newcommand{\Ga}{\alpha}
\newcommand{\Gb}{\beta}
\newcommand{\Gd}{\delta}
\newcommand{\Ge}{\epsilon}
\newcommand{\Gve}{\varepsilon}
\newcommand{\Gf}{\phi}
\newcommand{\Gvf}{\varphi}
\newcommand{\Gg}{\gamma}
\newcommand{\Gc}{\chi}
\newcommand{\Gi}{\iota}
\newcommand{\Gk}{\kappa}
\newcommand{\Gl}{\lambda}
\newcommand{\Gn}{\eta}
\newcommand{\Gm}{\mu}
\newcommand{\Gv}{\nu}
\newcommand{\Gp}{\pi}
\newcommand{\Gt}{\theta}
\newcommand{\Gvt}{\vartheta}
\newcommand{\Gr}{\rho}
\newcommand{\Gvr}{\varrho}
\newcommand{\Gs}{\sigma}
\newcommand{\Gvs}{\varsigma}
\newcommand{\Gj}{\tau}
\newcommand{\Gu}{\upsilon}
\newcommand{\Go}{\omega}
\newcommand{\Gx}{\xi}
\newcommand{\Gy}{\psi}
\newcommand{\Gz}{\zeta}
\newcommand{\GD}{\Delta}
\newcommand{\GF}{\Phi}
\newcommand{\GG}{\Gamma}
\newcommand{\GL}{\Lambda}
\newcommand{\GP}{\Pi}
\newcommand{\GT}{\Theta}
\newcommand{\GS}{\Sigma}
\newcommand{\GU}{\Upsilon}
\newcommand{\GO}{\Omega}
\newcommand{\GX}{\Xi}
\newcommand{\GY}{\Psi}

% Abbreviate definitions of bold greek symbols
\newcommand{\BGa}{\bfm\alpha}
\newcommand{\BGb}{\bfm\beta}
\newcommand{\BGd}{\bfm\delta}
\newcommand{\BGe}{\bfm\epsilon}
\newcommand{\BGve}{\bfm\varepsilon}
\newcommand{\BGf}{\bfm\phi}
\newcommand{\BGvf}{\bfm\varphi}
\newcommand{\BGg}{\bfm\gamma}
\newcommand{\BGc}{\bfm\chi}
\newcommand{\BGi}{\bfm\iota}
\newcommand{\BGk}{\bfm\kappa}
\newcommand{\BGl}{\bfm\lambda}
\newcommand{\BGn}{\bfm\eta}
\newcommand{\BGm}{\bfm\mu}
\newcommand{\BGv}{\bfm\nu}
\newcommand{\BGp}{\bfm\pi}
\newcommand{\BGt}{\bfm\theta}
\newcommand{\BGvt}{\bfm\vartheta}
\newcommand{\BGr}{\bfm\rho}
\newcommand{\BGvr}{\bfm\varrho}
\newcommand{\BGs}{\bfm\sigma}
\newcommand{\BGvs}{\bfm\varsigma}
\newcommand{\BGj}{\bfm\tau}
\newcommand{\BGu}{\bfm\upsilon}
\newcommand{\BGo}{\bfm\omega}
\newcommand{\BGx}{\bfm\xi}
\newcommand{\BMx}{\bfm\xi}
\newcommand{\BGy}{\bfm\psi}
\newcommand{\BGz}{\bfm\zeta}
\newcommand{\BGD}{\bfm\Delta}
\newcommand{\BGF}{\bfm\Phi}
\newcommand{\BGG}{\bfm\Gamma}
\newcommand{\BGL}{\bfm\Lambda}
\newcommand{\BGP}{\bfm\Pi}
\newcommand{\BGT}{\bfm\Theta}
\newcommand{\BGS}{\bfm\Sigma}
\newcommand{\BGU}{\bfm\Upsilon}
\newcommand{\BGO}{\bfm\Omega}
\newcommand{\BGX}{\bfm\Xi}
\newcommand{\BGY}{\bfm\Psi}

%Definitions: calligraphic letters
\newcommand{\mA}{\ensuremath{\mathcal{A}}}
\newcommand{\mB}{\ensuremath{\mathcal{B}}}
\newcommand{\mC}{\ensuremath{\mathcal{C}}}
\newcommand{\mD}{\ensuremath{\mathcal{D}}}
\newcommand{\mE}{\ensuremath{\mathcal{E}}}
\newcommand{\mF}{\ensuremath{\mathcal{F}}}
\newcommand{\mG}{\ensuremath{\mathcal{G}}}
\newcommand{\mH}{\ensuremath{\mathcal{H}}}
\newcommand{\mI}{\ensuremath{\mathcal{I}}}
\newcommand{\mJ}{\ensuremath{\mathcal{J}}}
\newcommand{\mK}{\ensuremath{\mathcal{K}}}
\newcommand{\mL}{\ensuremath{\mathcal{L}}}
\newcommand{\mM}{\ensuremath{\mathcal{M}}}
\newcommand{\mN}{\ensuremath{\mathcal{N}}}
\newcommand{\mO}{\ensuremath{\mathcal{O}}}
\newcommand{\mP}{\ensuremath{\mathcal{P}}}
\newcommand{\mQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\mR}{\ensuremath{\mathcal{R}}}
\newcommand{\mS}{\ensuremath{\mathcal{S}}}
\newcommand{\mT}{\ensuremath{\mathcal{T}}}
\newcommand{\mU}{\ensuremath{\mathcal{U}}}
\newcommand{\mV}{\ensuremath{\mathcal{V}}}
\newcommand{\mW}{\ensuremath{\mathcal{W}}}
\newcommand{\mX}{\ensuremath{\mathcal{X}}}
\newcommand{\mY}{\ensuremath{\mathcal{Y}}}
\newcommand{\mZ}{\ensuremath{\mathcal{Z}}}

%Definitions: bold calligraphic letters
\newcommand{\bmA}{\mbox{\boldmath $\mathcal{A}$}}
\newcommand{\bmB}{\mbox{\boldmath $\mathcal{B}$}}
\newcommand{\bmC}{\mbox{\boldmath $\mathcal{C}$}}
\newcommand{\bmD}{\mbox{\boldmath $\mathcal{D}$}}
\newcommand{\bmE}{\mbox{\boldmath $\mathcal{E}$}}
\newcommand{\bmF}{\mbox{\boldmath $\mathcal{F}$}}
\newcommand{\bmG}{\mbox{\boldmath $\mathcal{G}$}}
\newcommand{\bmH}{\mbox{\boldmath $\mathcal{H}$}}
\newcommand{\bmI}{\mbox{\boldmath $\mathcal{I}$}}
\newcommand{\bmJ}{\mbox{\boldmath $\mathcal{J}$}}
\newcommand{\bmK}{\mbox{\boldmath $\mathcal{K}$}}
\newcommand{\bmL}{\mbox{\boldmath $\mathcal{L}$}}
\newcommand{\bmM}{\mbox{\boldmath $\mathcal{M}$}}
\newcommand{\bmN}{\mbox{\boldmath $\mathcal{N}$}}
\newcommand{\bmO}{\mbox{\boldmath $\mathcal{O}$}}
\newcommand{\bmP}{\mbox{\boldmath $\mathcal{P}$}}
\newcommand{\bmQ}{\mbox{\boldmath $\mathcal{Q}$}}
\newcommand{\bmR}{\mbox{\boldmath $\mathcal{R}$}}
\newcommand{\bmS}{\mbox{\boldmath $\mathcal{S}$}}
\newcommand{\bmT}{\mbox{\boldmath $\mathcal{T}$}}
\newcommand{\bmU}{\mbox{\boldmath $\mathcal{U}$}}
\newcommand{\bmV}{\mbox{\boldmath $\mathcal{V}$}}
\newcommand{\bmW}{\mbox{\boldmath $\mathcal{W}$}}
\newcommand{\bmX}{\mbox{\boldmath $\mathcal{X}$}}
\newcommand{\bmY}{\mbox{\boldmath $\mathcal{Y}$}}
\newcommand{\bmZ}{\mbox{\boldmath $\mathcal{Z}$}}

%Definitions: functions
\DeclareMathOperator{\tr}{tr}
% \newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\dev}{\mathop{\mathrm{dev}}}
\newcommand{\diver}{\mathop{\mathrm{div}}}
\newcommand{\Div}{\mathop{\mathrm{Div}}}
\newcommand{\grad}{\mathop{\mathrm{grad}}}
\newcommand{\Grad}{\mathop{\mathrm{Grad}}}
\newcommand{\curl}{\mathop{\mathrm{curl}}}
\def\Im{\mathop{\mathrm{Im}}}
\def\Re{\mathop{\mathrm{Re}}}
\newcommand{\Ei}{\mathop{\mathrm{Ei}}}
\newcommand{\Ci}{\mathop{\mathrm{Ci}}}
\newcommand{\Si}{\mathop{\mathrm{Si}}}
\newcommand{\sign}{\mathop{\mathrm{sign}}}
\newcommand{\Res}{\mathop{\mathrm{Res}}}
\newcommand{\arctanh}{\mathop{\mathrm{arctanh}}}

%Definitions: sets
\def\Lin{\ensuremath{\mathsf{Lin}}}
\def\Orth{\ensuremath{\mathsf{Orth}}}
\def\Sym{\ensuremath{\mathsf{Sym}}}
\newcommand{\Reals}{\ensuremath{\mathbb{R}}}
\newcommand{\Complex}{\ensuremath{\mathbb{C}}}
\newcommand{\Naturals}{\ensuremath{\mathbb{N}}}

%Definitions: journals
\def\AAM{{\it Arch.\ Appl.\ Mech.}\ }
\def\ACIJ{{\it ACI J.}\ }
\def\ACISJ{{\it ACI Struct.\ J.}\ }
\def\ACSB{{\it Am.\ Ceram.\ Soc.\ Bull.}\ }
\def\AM{{\it Acta mater.}\ }
\def\AMPA{{\it Ann.\ Mat.\ Pur.\ Appl.}\ }
\def\AMR{{\it Appl.\ Mech.\ Rev.}\ }
\def\ARMA{{\it Arch.\ Ration.\ Mech.\ An.}\ }
\def\CACS{{\it Comm.\ Am.\ Cer.\ Soc.}\ }
\def\CMAME{{\it Comput.\ Method.\ Appl.\ M.}\ }
\def\EFM{{\it Eng.\ Fract.\ Mech.}\ }
\def\EJMA{{\it Eur.\ J.\ Mech. A-Solid.}\ }
\def\IA{{\it Ing.\ Arch.}\ }
\def\IMA{{\it IMA J.\ Appl.\ Math.}\ }
\def\IJES{{\it Int.\ J.\ Eng.\ Sci.}\ }
\def\IJF{{\it Int.\ J.\ Fracture}\ }
\def\IJMS{{\it Int.\ J.\ Mech.\ Sci.}\ }
\def\IJNAMG{{\it Int.\ J.\ Numer.\ Anal.\ Meth.\ Geomech.}\ }
\def\IJNME{{\it Int.\ J.\ Numer.\ Meth.\ Eng.}\ }
\def\IJP{{\it Int.\ J.\ Plasticity}\ }
\def\IJSS{{\it Int.\ J.\ Solids Struct.}\ }
\def\JACS{{\it J.\ Am.\ Ceram.\ Soc.}\ }
\def\JAM{{\it ASME J.\ Appl.\ Mech.}\ }
\def\JAP{{\it J.\ Appl.\ Phys.}\ }
\def\JE{{\it J.\ Elasticity}\ }
\def\JEM{{\it ASCE J.\ Eng.\ Mech.}\ }
\def\JEMD{{\it ASCE J.\ Eng.\ Mech.\ Div.}\ }
\def\JEMT{{\it ASME J.\ Eng.\ Mater.\ Tech.}\ }
\def\JM{{\it J.\ M\'ecanique}\ }
\def\JMPS{{\it J.\ Mech.\ Phys.\ Solids}\ }
\def\JSHA{{\it J.\ Soc.\ Hungarian Arch.}\ }
\def\MCFM{{\it Mech.\ Cohes-Frict.\ Mat.}\ }
\def\MCM{{\it Mech.\ Compos.\ Mater.}\ }
\def\MDPM{{\it Mod.\ Dev.\ Powder Metall.}\ }
\def\ME{{\it Mater.\ Eng.}\ }
\def\MMS{{\it Math.\ Mech.\ Solids}\ }
\def\MOM{{\it Mech.\ Materials}\ }
\def\MPCPS{{\it Math.\ Proc.\ Camb.\ Phil.\ Soc.}\ }
\def\MRC{{\it Mech.\ Res.\ Commun.}\ }
\def\MRSB{{\it MRS Bull.}\ }
\def\MSE{{\it Mater.\ Sci.\ Eng.}\ }
\def\NED{{\it Nucl.\ Eng.\ Des.}\ }
\def\PM{{\it Phil.\ Mag.}\ }
\def\PRSL{{\it Proc.\ R.\ Soc.\ Lond.}\ }
\def\QAM{{\it Quart.\ Appl.\ Math.}\ }
\def\QJMAM{{\it Quart.\ J.\ Mech.\ Appl.\ Math.}\ }
\def\SF{{\it Soils Found.}\ }
\def\ZAMP{{\it Z.\ Angew.\ Math.\ Phys.}\ }
\def\ZAMM{{\it Z.\ Angew.\ Math.\ Mech.}\ }
\def\ZP{{\it Z.\ Phys.}\ }

